The Effects of Diffuse Ionized Gas and Spatial Resolution on Metallicity Gradients: TYPHOON Two-Dimensional Spectrophotometry of M83

We present a systematic study of the diffuse ionized gas (DIG) in M83 and its effects on the measurement of metallicity gradients at varying resolution scales. Using spectrophotometric data cubes of M83 obtained at the 2.5m duPont telescope at Las Campanas Observatory as part of the TYPHOON program, we separate the HII regions from the DIG using the [SII]/H$\alpha$ ratio, HIIphot (HII finding algorithm) and the H$\alpha$ surface brightness. We find that the contribution to the overall H$\alpha$ luminosity is approximately equal for the HII and DIG regions. The data is then rebinned to simulate low-resolution observations at varying resolution scales from 41 pc up to 1005 pc. Metallicity gradients are measured using five different metallicity diagnostics at each resolution. We find that all metallicity diagnostics used are affected by the inclusion of DIG to varying degrees. We discuss the reasons of why the metallicity gradients are significantly affected by DIG using the HII dominance and emission line ratio radial profiles. We find that applying the [SII]/H$\alpha$ cut will provide a closer estimate of the true metallicity gradient up to a resolution of 1005 pc for all metallicity diagnostics used in this study.

==> commands.tex <==
\newcommand{\rtt}{$\textrm{R}_{23}$ }

\newcommand{\rtteq}{$(\textrm{[OII]} \lambda3726, \lambda3729+\textrm{[OIII]} \lambda4959, \lambda5007)$/$\textrm{H}\beta$ }

\newcommand{\mt}{$M_{20}$ }

\newcommand{\htwo}{H{\sc ii} }

\newcommand{\bpt}{Baldwin, Phillips and Terlevich (BPT) diagram \citep{baldwin81}}

\newcommand{\stha}{[SII]/H$\alpha$ }

\newcommand{\ntha}{[NII]/H$\alpha$ }

\newcommand{\angstrom}{\textup{\AA}}
